Point Process Modeling of Drug Overdoses with Heterogeneous and Missing Data

Opioid overdose rates have increased in the United States over the past decade and reflect a major public health crisis. Modeling and prediction of drug and opioid hotspots, where a high percentage of events fall in a small percentage of space-time, could help better focus limited social and health services. In this work we present a spatial-temporal point process model for drug overdose clustering. The data input into the model comes from two heterogeneous sources: 1) high volume emergency medical calls for service (EMS) records containing location and time, but no information on the type of non-fatal overdose and 2) fatal overdose toxicology reports from the coroner containing location and high-dimensional information from the toxicology screen on the drugs present at the time of death. We first use non-negative matrix factorization to cluster toxicology reports into drug overdose categories and we then develop an EM algorithm for integrating the two heterogeneous data sets, where the mark corresponding to overdose category is inferred for the EMS data and the high volume EMS data is used to more accurately predict drug overdose death hotspots. We apply the algorithm to drug overdose data from Indianapolis, showing that the point process defined on the integrated data outperforms point processes that use only homogeneous EMS (AUC improvement .72 to .8) or coroner data (AUC improvement .81 to .85).We also investigate the extent to which overdoses are contagious, as a function of the type of overdose, while controlling for exogenous fluctuations in the background rate that might also contribute to clustering. We find that drug and opioid overdose deaths exhibit significant excitation, with branching ratio ranging from .72 to .98.

==> Report 2/related_work.tex <==
\section{Related Work}
Point process models have been used 
to model earthquake occurrences since 1970s ~\cite{Ogata1999}. 
The epidemic-type aftershock sequence (ETAS) model, 
a branching process model in which all earthquakes can trigger aftershocks, 
has become one of the standard models in seismology~\cite{Ogata1988}~\cite{Ogata1998}. 
The branching process models are estimated using maximum likelihood (ML), 
with the use of expectation-maximization (EM) algorithm. 
The initial ETAS model was purely temporal, 
modeling the rate of earthquakes at time $t$ 
as a superposition of a constant rate of background seismicity and of aftershocks triggered by these background events: 
\begin{equation*}
\lambda(t) = \mu + \sum_{i: t_i < t} \frac{K_i}{(t-t_i+c)^p}.
\end{equation*}

Here $\mu$ is the background seismic activity rate 
and $K_i$ is related to the recorded magnitude $M_i$ of earthquake $i$ 
by the relationship $K_i = K_0 e^{\alpha (M_i-M_0)}$, 
where $M_0$ is the minimum magnitude threshold for earthquakes to be recorded in the dataset, and $K_0, \alpha, p$ are constants. \\

The ETAS models had been extended and takes the form 
\begin{equation*}
    \lambda(t,x,y) = \mu(x,y) + \sum_{i:t_i<t} g(t-t_i, x-x_i, y-y_i;M_i),
\end{equation*}
where mark $M_i$ is the magnitude of the earthquake associated with event $i$. 
In \cite{Ogata1998}, the kernel is estimated using
\begin{equation*}
    g(t,x,y;M) = \frac{K_0}{(t+c)^p} \cdot \frac{e^{\alpha(M-M_0)}}{(x^2+y^2+d)^q}.
\end{equation*}

After the development of ETAS models, 
~\cite{Mohler2011} drew an analogy between aftershock models and crime. Criminological theories suggest a model of crime which assumes the conditional intensity of crime occurrence can be divided into a chronic background portion, which may vary in space depending on a variety of factors, 
and a self-exciting portion which accounts for near-repeats and retaliations ~\cite{Mohler2011}:
\begin{equation}
\lambda(s,t) = \nu(t)\mu(s) + \sum_{i:t_i<t} g(s-s_i, t-t_i),
\label{general}
\end{equation}
where $g$ is a triggering function and $\mu(s)$, 
$\nu(t)$ reflects spatial and temporal changes from weather, seasonality, and so on.

To estimate the parameters in function \ref{general}, 
it is most common to use maximum likelihood estimation, 
where the log likelihood function \cite{Daley2003}
\begin{equation}
\begin{aligned}
    l(\theta) = \sum_k \text{log}&\left\{ \lambda(t_k, x_k, y_k;\theta)\right\}- \\
&\int_0^T\iint_S \lambda(t,x,y;\theta)dydxdt
\end{aligned}
\label{loglike}
\end{equation}
is maximized over all parameter sets $\theta$. 
Here $ S \times [0,T]$ is the space–time window of observation.\\

In this project, equation \ref{general} is rewritten with respect to location $(x,y)$ and time $t$
\begin{equation}
\lambda(x,y,t) = \mu_0 u(x,y)v(t) + \sum_{i:t_i<t} g(x-x_i, y-y_i, t-t_i),
\label{lambda}
\end{equation}

where $g$ is modelled as follows:
\begin{equation}
\begin{aligned}
g(x,y,t) =& \sum_{t>t_i}  K_{0} \left(w\cdot \text{exp}\left\{-w(t-t_i)\right\}\right) \cdot \\
& \frac{1}{{2\pi \sigma^2}}\cdot \text{exp} \left\{-\frac{1}{2\sigma^2} \left[ (x-x_i)^2 + (y-y_i)^2\right]\right\},
\end{aligned}
\label{trigger}
\end{equation}

Here, $\mu_0$ is the estimated number of background events, 
$K_0$ is the expected proportion of triggered events, 
$w^{-1}$ is the expected time interval of two triggered events, 
and $\sigma$ is expected distance between two triggered events.\\

In the next section, we will explain how the parameters are estimated and how the self-exciting point process is extended by adding labelled groups. 
Results of the experiments will be shown in section III. 
Conclusion and future work will be discussed in section IV.

==> related_work.tex <==
\section{Related Work}
Point process models have been used 
to model earthquake occurrences since 1970s ~\cite{Ogata1999}. 
The epidemic-type aftershock sequence (ETAS) model, 
a branching process model in which all earthquakes can trigger aftershocks, 
has become one of the standard models in seismology~\cite{Ogata1988}~\cite{Ogata1998}. 
The branching process models are estimated using maximum likelihood (ML), 
with the use of expectation-maximization (EM) algorithm. 
The initial ETAS model was purely temporal, 
modeling the rate of earthquakes at time $t$ 
as a superposition of a constant rate of background seismicity and of aftershocks triggered by these background events: 
\begin{equation*}
\lambda(t) = \mu + \sum_{i: t_i < t} \frac{K_i}{(t-t_i+c)^p}.
\end{equation*}

Here $\mu$ is the background seismic activity rate 
and $K_i$ is related to the recorded magnitude $M_i$ of earthquake $i$ 
by the relationship $K_i = K_0 e^{\alpha (M_i-M_0)}$, 
where $M_0$ is the minimum magnitude threshold for earthquakes to be recorded in the dataset, and $K_0, \alpha, p$ are constants. \\

The ETAS models had been extended and takes the form 
\begin{equation*}
    \lambda(t,x,y) = \mu(x,y) + \sum_{i:t_i<t} g(t-t_i, x-x_i, y-y_i;M_i),
\end{equation*}
where mark $M_i$ is the magnitude of the earthquake associated with event $i$. 
In \cite{Ogata1998}, the kernel is estimated using
\begin{equation*}
    g(t,x,y;M) = \frac{K_0}{(t+c)^p} \cdot \frac{e^{\alpha(M-M_0)}}{(x^2+y^2+d)^q}.
\end{equation*}

After the development of ETAS models, 
~\cite{Mohler2011} drew an analogy between aftershock models and crime. Criminological theories suggest a model of crime which assumes the conditional intensity of crime occurrence can be divided into a chronic background portion, which may vary in space depending on a variety of factors, 
and a self-exciting portion which accounts for near-repeats and retaliations ~\cite{Mohler2011}:
\begin{equation}
\lambda(s,t) = \nu(t)\mu(s) + \sum_{i:t_i<t} g(s-s_i, t-t_i),
\label{general}
\end{equation}
where $g$ is a triggering function and $\mu(s)$, 
$\nu(t)$ reflects spatial and temporal changes from weather, seasonality, and so on.

To estimate the parameters in function \ref{general}, 
it is most common to use maximum likelihood estimation, 
where the log likelihood function \cite{Daley2003}
\begin{equation}
\begin{aligned}
    l(\theta) = \sum_k \text{log}&\left\{ \lambda(t_k, x_k, y_k;\theta)\right\}- \\
&\int_0^T\iint_S \lambda(t,x,y;\theta)dydxdt
\end{aligned}
\label{loglike}
\end{equation}
is maximized over all parameter sets $\theta$. 
Here $ S \times [0,T]$ is the space–time window of observation.\\

In this project, equation \ref{general} is rewritten with respect to location $(x,y)$ and time $t$
\begin{equation}
\lambda(x,y,t) = \mu_0 u(x,y)v(t) + \sum_{i:t_i<t} g(x-x_i, y-y_i, t-t_i),
\label{lambda}
\end{equation}

where $g$ is modelled as follows:
\begin{equation}
\begin{aligned}
g(x,y,t) =& \sum_{t>t_i}  K_{0} \left(w\cdot \text{exp}\left\{-w(t-t_i)\right\}\right) \cdot \\
& \frac{1}{{2\pi \sigma^2}}\cdot \text{exp} \left\{-\frac{1}{2\sigma^2} \left[ (x-x_i)^2 + (y-y_i)^2\right]\right\},
\end{aligned}
\label{trigger}
\end{equation}

Here, $\mu_0$ is the estimated number of background events, 
$K_0$ is the expected proportion of triggered events, 
$w^{-1}$ is the expected time interval of two triggered events, 
and $\sigma$ is expected distance between two triggered events.\\

In the next section, we will explain how the parameters are estimated and how the self-exciting point process is extended by adding labelled groups. 
Results of the experiments will be shown in section III. 
Conclusion and future work will be discussed in section IV.
